Packing and emergence of ordering of rods in a spherical monolayer

Spatially ordered systems confined to surfaces such as spheres exhibit interesting topological structures because of curvature induced frustration in orientational as well as translational order. The study of these structures is important for investigating the interplay between geometry, topology, and elasticity, and for their potential applications in materials science. In this work we numerically simulate a spherical monolayer of soft repulsive spherocylinders (SRS) and study the packing of rods and their ordering transition as a function of the packing fraction. In the model that we study, centers of mass of the spherocylinders (situated at their geometric centers) are constrained to move on a spherical surface. The spherocylinders are free to rotate about any axis that passes through their respective centers of mass. We show that at relatively lower packing fractions, there is a continuous transition from a disordered fluid to a novel, orientationally ordered, spherical fluid monolayer as the packing fractions is increased. This monolayer of orientationally ordered SRS particles resembles a hedgehog -- long axes of the SRS particles are aligned along the local normal to the sphere. At higher packing fractions, system undergoes transition to the solid phase, which is riddled with topological point defects (disclinations) and grain boundaries that divide the whole surface into several domains.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

